Leveraging Knowledge in Multilingual Commonsense Reasoning

Commonsense reasoning (CSR) requires the model to be equipped with general world knowledge. While CSR is a language-agnostic process, most comprehensive knowledge sources are in few popular languages, especially English. Thus, it remains unclear how to effectively conduct multilingual commonsense reasoning (XCSR) for various languages. In this work, we propose to utilize English knowledge sources via a translate-retrieve-translate (TRT) strategy. For multilingual commonsense questions and choices, we collect related knowledge via translation and retrieval from the knowledge sources. The retrieved knowledge is then translated into the target language and integrated into a pre-trained multilingual language model via visible knowledge attention. Then we utilize a diverse of 4 English knowledge sources to provide more comprehensive coverage of knowledge in different formats. Extensive results on the XCSR benchmark demonstrate that TRT with external knowledge can significantly improve multilingual commonsense reasoning in both zero-shot and translate-train settings, outperforming 3.3 and 3.6 points over the previous state-of-the-art on XCSR benchmark datasets (X-CSQA and X-CODAH).

==> tables/datasets_copy.tex <==
\begin{table}[t!]
%\begin{adjustbox}{scale=0.8,center}
%\resizebox{1.0\columnwidth}{!}{
\small 
\begin{tabular}{lccc}
\toprule
% Dataset  & Task & \#train & \#dev & \#test & \#l \\
% \midrule
% X-CSQA & Question Answering & 8888 & 1000 & 1074 & 16 \\
% X-CODAH & Scene Completion & 8476 & 300 & 1000 & 7 \\
% XCOPA & Casual Reasoning & - & - & - & - \\

Dataset & X-CSQA & X-CODAH & XCOPA \\
\midrule
Task Format & QA & SceneComp. & CasualRea. \\
\#Languages & 16 & 16 & 12 \\
\#Options & 5 & 4 & 2 \\
\#train & 8888 & 8476 & 400 \\
\#dev & 1000 & 300 & 100 \\
\#test & 1074 & 1000 & 500 \\
\bottomrule
\end{tabular}
%\end{adjustbox}
\caption{Statistics of the three datasets for multilingual commonsense reasoning}
\label{tbl:stat}
% Struct. pred.: Structured prediction.
\end{table}

==> tables/gpt3.tex <==
\begin{table}[t!]
%\begin{adjustbox}{scale=0.95,center}
\resizebox{1.0\columnwidth}{!}{
\small
\begin{tabular}{l|c|ccc}
\toprule
& MCP & + Def. & + Triple. & + Sentence \\
\midrule
% \midrule
X-CSQA & 55.1 & 55.3 (57.0) & (55.4) &  (56.2) \\
X-CODAH & 57.9 & 59.1 (60.6) & 59.9 (60.4) & 58.4 (59.7) \\
\bottomrule
\end{tabular}
}
%\end{adjustbox}
\caption{Results of using GPT-3 to generate different knowledge format. The numbers in the bracket are the average accuracy of Wiktionary, ConceptNet and OMCS from Table~\ref{tbl:xcsr_full_dev} zero-shot transfer setting.}
\label{tbl:gpt3}
% Struct. pred.: Structured prediction.
\end{table}

==> tables/xcsqa_kg.tex <==
\begin{table*}[t!]
\centering
\resizebox{\linewidth}{!}{
\small 
\begin{tabular}{l|cccccccccccccccc|c}
\toprule
Model & en & de & it & es & fr & nl & ru & vi & zh & hi & pl & ar & ja & pt & sw & ur & avg \\
\midrule
\multicolumn{18}{l}{\textit{Zero-shot transfer (models are trained on English data) and evaluate on the target language}} \\
\midrule
XLM-R-L                     & 68.3 & 57.4 & 55.5 & 57.2 & 56.6 & 57.2 & 55.2 & 53.4 & 55.9 & 49.6 & 54.2 & 51.9 & 48.5 & 56.0 & 40.0 & 46.4 & 54.0 \\
MCP               & 69.2 & 58.4 & 58 & 58.8 & 59.3 & 56 & 54.4 & 55.3 & 57.9 & 48.5 & 54.8 & 52.3 & 52.8 & 57.5 & 40.7 & 48.6 & 55.2 \\ \midrule
+ ConceptNet & 71.7 & 57.9 & 54.7 & 56.6 & 56.3 & 54.8 & 51.2 & 52.1 & 52.9 & 47.4 & 52.5 & 51.2 & 49.1 & 58.6 & 41.6 & 42 & 53.2 \\
+ IR & 71.2 & 57.4 & 57.5 & 60.2 & 57.3 & 58 & 56.5 & 58.5 & 58.4 & 50 & 55.6 & 53.2 & 53.2 & 57.4 & 46.5 & 47.7 & 56.2 \\ 
+ Dict & 70.9 & 60.7 & 59.3 & 59.8 & 60 & 59.5 & 55.4 & 57.3 & 58.9 & 50.8 & 57.5 & 54.6 & 50.8 & 60.9 & 47.1 & 50.2 & 57.1 \\
%+ GPT-3               & 69.5 & 59.3 & 60.3 & 61.4 & 60.0 & 61.1 & 57.5 & 55.7 & 56.7 & 51.3 & 56.1 & 52.3 & 50.2 & 60.7 & 43.3 & 48.8 & 56.5 \\
\midrule
%\multicolumn{18}{l}{\textit{Translate-test (models are trained on English data and evaluated on target language data translated to English)}} \\
\multicolumn{18}{l}{\textit{Zero-shot transfer and evaluate on target language data translated to English}} \\
\midrule 
XLM-R-L & 68.3 & 60.1 & 56.9 & 60.9 & 58.8 & 58.7 & 56.9 & 56.9 & 51.7 & 49.7 & 58.8 & 53.1 & 52.6 & 59.6 & 51 & 52.1 & 56.6 \\
MCP & 69.2 & 61.9 & 60.1 & 63.3 & 60.5 & 58.7 & 57.7 & 57.3 & 52.8 & 51.2 & 58.5 & 55.1 & 51.7 & 61.8 & 52 & 52.5 & 57.8 \\ \midrule
+ ConceptNet & 71.7 & 59.5 & 58.8 & 61.4 & 61.1 & 57.5 & 55.8 & 54.7 & 51.9 & 47 & 58.6 & 53.4 & 49.4 & 60.3 & 51.5 & 49.9 & 56.4 \\
+ IR & 71.2 & 60.8 & 59.3 & 63.2 & 61.7 & 59.7 & 57.9 & 57 & 51.7 & 50 & 60.5 & 55.5 & 51.2 & 62.3 & 52.8 & 53.5 & 58 \\ 
+ Dict & 70.9 & 63.2 & 61.5 & 62.9 & 62.1 & 60.1 & 60.1 & 57.9 & 52.9 & 50.9 & 60.7 & 54 & 52 & 61 & 54.7 & 54.4 & 58.7 \\
\midrule \midrule
\multicolumn{18}{l}{\textit{Translate-train (models are trained on English training data and its translated data) and evaluate on the target language}} \\
\midrule 
XLM-R-L & 66.7 & 60.2 & 58.5 & 60.4 & 58.6 & 56.4 & 56.3 & 57 & 57.4 & 50.9 & 56.2 & 53.8 & 54.3 & 59.2 & 47.5 & 48 & 56.3 \\
MCP & 69.2 & 60.2 & 59.2 & 60.2 & 58.8 & 59.1 & 57.5 & 60.2 & 57.8 & 51.2 & 57.6 & 56.5 & 54.6 & 59.4 & 47.4 & 51 & 57.5 \\ \midrule
+ ConceptNet & 73.3 & 58.7 & 58.8 & 58.4 & 58.9 & 56 & 55.3 & 53.1 & 55 & 48.3 & 56.9 & 51 & 51.7 & 59 & 43.4 & 45.5 & 55.2 \\ 
+ IR & 71.7 & 61.3 & 61.2 & 62.2 & 59.6 & 59.1 & 57 & 57.8 & 58.3 & 51.3 & 58.9 & 55.4 & 54.3 & 60.7 & 48.2 & 51.5 & 58 \\
+ Dict & 68.2 & 61.3 & 62.4 & 61.8 & 61.4 & 60.2 & 57.6 & 60.1 & 60.5 & 52.9 & 59.1 & 58.7 & 55.7 & 60.3 & 51.1 & 54.4 & 59.1 \\
\midrule
\multicolumn{18}{l}{\textit{Translate-train and evaluate on target language data translated to English}} \\
\midrule
XLM-R-L & 66.7 & 61.1 & 60.8 & 62.5 & 58.7 & 59.1 & 56.8 & 56.8 & 52 & 51.7 & 59.6 & 56.5 & 52.6 & 60.9 & 53.5 & 55.6 & 57.8 \\
MCP & 69.2 & 62 & 60.6 & 61.3 & 61 & 59.1 & 58.2 & 59.8 & 54.5 & 52.2 & 59.7 & 56.4 & 53.3 & 61.3 & 54.7 & 55.6 & 58.7 \\ \midrule
+ ConceptNet & 73.3 & 60.7 & 60 & 61.4 & 61.8 & 58.2 & 57.5 & 54.8 & 51.9 & 49.1 & 58.3 & 54.5 & 48.7 & 61.8 & 51.1 & 50.2 & 57.1 \\
+ IR & 71.7 & 63.3 & 62.6 & 63 & 62.3 & 61 & 60.6 & 58.5 & 52.8 & 52.1 & 60.3 & 56 & 51.5 & 61.2 & 55 & 56.7 & 59.3 \\
+ Dict & 69.4 & 62.1 & 62.5 & 62.7 & 64.6 & 62.1 & 59.4 & 61 & 58 & 52.8 & 60.8 & 57.2 & 53.4 & 62.7 & 53.9 & 56.8 & 60 \\


\bottomrule
\end{tabular}
}
\caption{XCSQA dev results.}
\label{tbl:xcsr}
%\vspace{-1mm}
\end{table*}\begin{table*}[t!]
\centering
\resizebox{\linewidth}{!}{
\small 
\begin{tabular}{l|cccccccccccccccc|c}
\toprule
Model & en & de & it & es & fr & nl & ru & vi & zh & hi & pl & ar & ja & pt & sw & ur & avg \\
\midrule
\multicolumn{18}{l}{\textit{Zero-shot transfer (models are trained on English data) and evaluate on the target language}} \\
\midrule
XLM-R-L                     & 68.3 & 57.4 & 55.5 & 57.2 & 56.6 & 57.2 & 55.2 & 53.4 & 55.9 & 49.6 & 54.2 & 51.9 & 48.5 & 56.0 & 40.0 & 46.4 & 54.0 \\
MCP               & 69.2 & 58.4 & 58 & 58.8 & 59.3 & 56 & 54.4 & 55.3 & 57.9 & 48.5 & 54.8 & 52.3 & 52.8 & 57.5 & 40.7 & 48.6 & 55.2 \\ \midrule
+ ConceptNet & 71.7 & 57.9 & 54.7 & 56.6 & 56.3 & 54.8 & 51.2 & 52.1 & 52.9 & 47.4 & 52.5 & 51.2 & 49.1 & 58.6 & 41.6 & 42 & 53.2 \\
+ IR & 71.2 & 57.4 & 57.5 & 60.2 & 57.3 & 58 & 56.5 & 58.5 & 58.4 & 50 & 55.6 & 53.2 & 53.2 & 57.4 & 46.5 & 47.7 & 56.2 \\ 
+ Dict & 70.9 & 60.7 & 59.3 & 59.8 & 60 & 59.5 & 55.4 & 57.3 & 58.9 & 50.8 & 57.5 & 54.6 & 50.8 & 60.9 & 47.1 & 50.2 & 57.1 \\
%+ GPT-3               & 69.5 & 59.3 & 60.3 & 61.4 & 60.0 & 61.1 & 57.5 & 55.7 & 56.7 & 51.3 & 56.1 & 52.3 & 50.2 & 60.7 & 43.3 & 48.8 & 56.5 \\
\midrule
%\multicolumn{18}{l}{\textit{Translate-test (models are trained on English data and evaluated on target language data translated to English)}} \\
\multicolumn{18}{l}{\textit{Zero-shot transfer and evaluate on target language data translated to English}} \\
\midrule 
XLM-R-L & 68.3 & 60.1 & 56.9 & 60.9 & 58.8 & 58.7 & 56.9 & 56.9 & 51.7 & 49.7 & 58.8 & 53.1 & 52.6 & 59.6 & 51 & 52.1 & 56.6 \\
MCP & 69.2 & 61.9 & 60.1 & 63.3 & 60.5 & 58.7 & 57.7 & 57.3 & 52.8 & 51.2 & 58.5 & 55.1 & 51.7 & 61.8 & 52 & 52.5 & 57.8 \\ \midrule
+ ConceptNet & 71.7 & 59.5 & 58.8 & 61.4 & 61.1 & 57.5 & 55.8 & 54.7 & 51.9 & 47 & 58.6 & 53.4 & 49.4 & 60.3 & 51.5 & 49.9 & 56.4 \\
+ IR & 71.2 & 60.8 & 59.3 & 63.2 & 61.7 & 59.7 & 57.9 & 57 & 51.7 & 50 & 60.5 & 55.5 & 51.2 & 62.3 & 52.8 & 53.5 & 58 \\ 
+ Dict & 70.9 & 63.2 & 61.5 & 62.9 & 62.1 & 60.1 & 60.1 & 57.9 & 52.9 & 50.9 & 60.7 & 54 & 52 & 61 & 54.7 & 54.4 & 58.7 \\
\midrule \midrule
\multicolumn{18}{l}{\textit{Translate-train (models are trained on English training data and its translated data) and evaluate on the target language}} \\
\midrule 
XLM-R-L & 66.7 & 60.2 & 58.5 & 60.4 & 58.6 & 56.4 & 56.3 & 57 & 57.4 & 50.9 & 56.2 & 53.8 & 54.3 & 59.2 & 47.5 & 48 & 56.3 \\
MCP & 69.2 & 60.2 & 59.2 & 60.2 & 58.8 & 59.1 & 57.5 & 60.2 & 57.8 & 51.2 & 57.6 & 56.5 & 54.6 & 59.4 & 47.4 & 51 & 57.5 \\ \midrule
+ ConceptNet & 73.3 & 58.7 & 58.8 & 58.4 & 58.9 & 56 & 55.3 & 53.1 & 55 & 48.3 & 56.9 & 51 & 51.7 & 59 & 43.4 & 45.5 & 55.2 \\ 
+ IR & 71.7 & 61.3 & 61.2 & 62.2 & 59.6 & 59.1 & 57 & 57.8 & 58.3 & 51.3 & 58.9 & 55.4 & 54.3 & 60.7 & 48.2 & 51.5 & 58 \\
+ Dict & 68.2 & 61.3 & 62.4 & 61.8 & 61.4 & 60.2 & 57.6 & 60.1 & 60.5 & 52.9 & 59.1 & 58.7 & 55.7 & 60.3 & 51.1 & 54.4 & 59.1 \\
\midrule
\multicolumn{18}{l}{\textit{Translate-train and evaluate on target language data translated to English}} \\
\midrule
XLM-R-L & 66.7 & 61.1 & 60.8 & 62.5 & 58.7 & 59.1 & 56.8 & 56.8 & 52 & 51.7 & 59.6 & 56.5 & 52.6 & 60.9 & 53.5 & 55.6 & 57.8 \\
MCP & 69.2 & 62 & 60.6 & 61.3 & 61 & 59.1 & 58.2 & 59.8 & 54.5 & 52.2 & 59.7 & 56.4 & 53.3 & 61.3 & 54.7 & 55.6 & 58.7 \\ \midrule
+ ConceptNet & 73.3 & 60.7 & 60 & 61.4 & 61.8 & 58.2 & 57.5 & 54.8 & 51.9 & 49.1 & 58.3 & 54.5 & 48.7 & 61.8 & 51.1 & 50.2 & 57.1 \\
+ IR & 71.7 & 63.3 & 62.6 & 63 & 62.3 & 61 & 60.6 & 58.5 & 52.8 & 52.1 & 60.3 & 56 & 51.5 & 61.2 & 55 & 56.7 & 59.3 \\
+ Dict & 69.4 & 62.1 & 62.5 & 62.7 & 64.6 & 62.1 & 59.4 & 61 & 58 & 52.8 & 60.8 & 57.2 & 53.4 & 62.7 & 53.9 & 56.8 & 60 \\


\bottomrule
\end{tabular}
}
\caption{XCSQA dev results.}
\label{tbl:xcsr}
%\vspace{-1mm}
\end{table*}

==> tables/xcsr_tt.tex <==
\begin{table*}[t!]
\centering
\resizebox{\linewidth}{!}{
\small 
\begin{tabular}{l|c|cccccccccccccccc|c}
\toprule
Dataset & Model & en & de & it & es & fr & nl & ru & vi & zh & hi & pl & ar & ja & pt & sw & ur & avg \\
\midrule
%\multicolumn{18}{c}{X-CSQA} \\
%\multirow{5}{*}{X-CSQA} & XLMR-L & 66.7 & 60.2 & 58.5 & 60.4 & 58.6 & 56.4 & 56.3 & 57 & 57.4 & 50.9 &  56.2 & 53.8 & 54.3 & 592 & 47.5 & 48 & 56.3 \\
%& \enspace + Cpnt & 71.7 & 57.9 & 54.7 & 56.6 & 56.3 & 54.8 & 51.2 & 52.1 & 52.9 & 47.4 & 52.5 & 51.2 & 49.1 & 58.6 & 41.6 & 42 & 53.2 \\
\multirow{4}{*}{X-CSQA} & MCP (RL) & 69.4 & 59.3 & 60.6 & 60.9 & 60.8 & 57.9 & 57.0 & 58.2 & 58.0 & 50.4 & 58.3 & 55.1 & 53.9 & 60.3 & 47.1 & 50.9 & 57.4 \\
\cmidrule{2-19}
& \enspace + Wikt. & 70.0 & 61.7 & 61.2 & 61.1 & 60.9 & 59.8 & 59.8 & 59.3 & 59.6 & 53.8 & 59.7 & 58.1 & 54.3 & 60.5 & 51.8 & 52.8 & 59.0 \\
& \enspace + Cpnt. & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
& \enspace + OMCS & 71.7 & 61.1 & 63.6 & 62.8 & 60.3 & 58.6 & 58.1 & 59.3 & 58.5 & 51.7 & 58.1 & 56.1 & 54.2 & 60.4 & 48.6 & 53.4 & 58.5 \\

%+ GPT-3               & 69.5 & 59.3 & 60.3 & 61.4 & 60.0 & 61.1 & 57.5 & 55.7 & 56.7 & 51.3 & 56.1 & 52.3 & 50.2 & 60.7 & 43.3 & 48.8 & 56.5 \\
\midrule \midrule
%\multicolumn{18}{c}{X-CODAH} \\
%\midrule 
%\multirow{6}{*}{X-CODAH} & XLMR-L & 72.0 & 71.0 & 66.3 & 68.3 & 70.0 & 66.0 & 61.7 & 61.7 & 63.7 & 60.3 & 67.3 & 60.0 & 60.3 & 68.0 & 57.0 & 57.0 & 64.4 \\
& MCP (RL) & 71.0 & 70.7 & 67.3 & 67.7 & 66.7 & 67.7 & 65.3 & 61.3 & 65.3 & 59.3 & 64.7 & 58.7 & 63.7 & 62.7 & 53.0 & 56.0 & 63.8 \\
\cmidrule{2-19}
\multirow{4}{*}{X-CODAH} & \enspace + Wikt. & 73.0 & 70.3 & 68.7 & 67.7 & 70.3 & 68.0 & 64.3 & 63.7 & 63.0 & 58.7 & 64.7 & 59.0 & 62.0 & 66.7 & 57.0 & 59.7 & 64.8 \\
& \enspace + Cpnt. & 70.0 & 68.7 & 68.7 & 67.7 & 66.7 & 68.3 & 62.7 & 63.0 & 63.0 & 59.0 & 65.0 & 60.3 & 61.0 & 67.7 & 62.0 & 59.7 & 64.6 \\
& \enspace + OMCS. & 74.7 & 69.7 & 67.3 & 67.7 & 67.7 & 68.3 & 62.7 & 65.3 & 65.3 & 58.7 & 68.3 & 62.0 & 64.0 & 68.3 & 56.7 & 59.7 & 65.4 \\
% \midrule
% \midrule \midrule
% & & en & et	& ht & id & it & qu & sw & ta & th & tr & vi & zh & - & - & - & - & avg \\
% \multirow{5}{*}{XCOPA} & XLMR-L & &  - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% \cmidrule{2-19}
% & \enspace + Wikt. &  - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% & \enspace + Cpnt. &  - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% & \enspace + OMCS &  - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
}
\caption{
Comparisons for TRT with different knowledge sources in the translate-train setting which are trained on English training data and its translated data. We use Microsoft Machine Translator to translate the English training data to all target languages in each dataset. The GPT-3 results are ommited to save time and budget because of its comparable performances over the baseline in Table~\ref{tbl:xcsr_zs_dev}.}
\label{tbl:xcsr_tt_dev}
%\vspace{-1mm}
\end{table*}

==> tables/xcsr_zs.tex <==
\begin{table*}[t!]
\centering
\resizebox{\linewidth}{!}{
\small 
\begin{tabular}{l|c|cccccccccccccccc|c}
\toprule
Dataset & Model & en & de & it & es & fr & nl & ru & vi & zh & hi & pl & ar & ja & pt & sw & ur & avg \\
\midrule
%\multicolumn{18}{c}{X-CSQA} \\
%\multirow{6}{*}{X-CSQA} & XLMR-L & 68.3 & 57.4 & 55.5 & 57.2 & 56.6 & 57.2 & 55.2 & 53.4 & 55.9 & 49.6 & 54.2 & 51.9 & 48.5 & 56.0 & 40.0 & 46.4 & 54.0 \\
\multirow{5}{*}{X-CSQA} & MCP (RL) & 69.0 & 57.6 & 57.2 & 57.9 & 59.9 & 56.1 & 55.2 & 56.0 & 56.6 & 48.8 & 56.4 & 52.5 & 50.8 & 58.3 & 42.5 & 47.4 & 55.1 \\
\cmidrule{2-19}
& \enspace + Wikt. & 70.7 & 59.5 & 60.2 & 61.4 & 59.5 & 58.5 & 56.6 & 55.6 & 58.3 & 51.2 & 56.0 & 55.6 & 52.0 & 60.6 & 46.8 & 49.1 & 57.0 \\
& \enspace + Cpnt. & 70.7 & 57.2 & 58.1 & 58.6 & 58.7 & 55.8 & 55.5 & 56.0 & 56.6 & 49.9 & 55.9 & 53.9 & 52.4 & 55.6 & 43.3 & 47.8 & 55.4 \\
& \enspace + OMCS & 70.5 & 59.9 & 59.3 & 60.5 & 60.0 & 56.8 & 55.3 & 56.1 & 57.3 & 48.9 & 56.4 & 53.4 & 51.6 & 59.0 & 46.7 & 48.0 & 56.2 \\
& \enspace + GPT-3 & 70.3 & 57.2 & 58.8 & 60.2 & 58.3 & 58.1 & 54.8 & 55.0 & 55.6 & 49.0 & 54.5 & 52.9 & 52.1 & 57.9 & 42.9 & 47.6 & 55.3 \\
%+ GPT-3               & 69.5 & 59.3 & 60.3 & 61.4 & 60.0 & 61.1 & 57.5 & 55.7 & 56.7 & 51.3 & 56.1 & 52.3 & 50.2 & 60.7 & 43.3 & 48.8 & 56.5 \\
\midrule \midrule
%\multicolumn{18}{c}{X-CODAH} \\
%\multirow{6}{*}{X-CODAH} & XLMR-L & 66.7 & 60.2 & 58.5 & 60.4 & 58.6 & 56.4 & 56.3 & 57 & 57.4 & 50.9 & 56.2 & 53.8 & 54.3 & 59.2 & 47.5 & 48 & 56.3 \\
\multirow{5}{*}{X-CODAH} & MCP (RL) & 69.7 & 63.0 & 62.3 & 63.0 & 64.7 & 64.7 & 55.0 & 55.0 & 59.7 & 54.3 & 61.7 & 52.3 & 57.0 & 55.0 & 40.3 & 49.3 & 57.9 \\ 
\cmidrule{2-19}
& \enspace + Wikt. & 71.0 & 64.7 & 66.0 & 66.0 & 63.0 & 60.7 & 56.7 & 57.7 & 59.0 & 56.0 & 62.3 & 52.3 & 59.7 & 59.7 & 41.3 & 55.0 & 59.4 \\
& \enspace + Cpnt. & 72.3 & 68.3 & 65.7 & 65.0 & 66.0 & 64.3 & 60.3 & 57.0 & 58.3 & 55.0 & 65.3 & 53.7 & 57.3 & 59.7 & 46.3 & 52.0 & 60.4 \\ 
& \enspace + OMCS & 73.0 & 67.0 & 64.0 & 63.7 & 63.0 & 62.0 & 57.3 & 60.0 & 62.0 & 53.0 & 63.7 & 56.0 & 57.7 & 59.3 & 44.0 & 49.3 & 59.7 \\
& \enspace + GPT-3 & 69.7 & 65.0 & 60.7 & 62.7 & 65.0 & 62.7 & 57.0 & 54.7 & 58.0 & 53.7 & 63.7 & 51.3 & 57.7 & 55.3 & 41.0 & 50.0 & 58.0 \\
% \midrule \midrule
% & & en & et	& ht & id & it & qu & sw & ta & th & tr & vi & zh & - & - & - & - & avg \\
% \multirow{5}{*}{XCOPA} & XLMR-L &  - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% \cmidrule{2-19}
% & \enspace + Wikt. &  - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% & \enspace + Cpnt. &  - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% & \enspace + OMCS &  - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% & \enspace + GPT-3 &  - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
}
\caption{Comparisons for TRT with different knowledge sources in the zero-shot setting which are trained on the English training data. We report results on development set for X-CSQA and X-CODAH to avoid multiple leaderboard submissions.
%For XCOPA, the results are evaluate on the public test set. XLMR-L and MCP (RL) and our reproduced results. Wikt. and Cpnt. are short for Wiktionary and ConceptNet respectively.
%For XCOPA, we sequentially fine-tune SocialIQA and COPA as the SI+CO-ZS setup in~\cite{xcopa}.
}
\label{tbl:xcsr_zs_dev}
%\vspace{-1mm}
\end{table*}

==> tables/xglue_leaderboard.tex <==
\begin{table*}[t!]
\centering
%\begin{adjustbox}{scale=0.95,center}
\small
\begin{tabular}{lcccccccccc}
\toprule

Model & Avg & NER & POS	& NC & MLQA & XNLI & PAWS-X & QADSM & WPR & QAM \\
\midrule
Unicoder & 76.1 & 79.7 & 79.6	& \textbf{83.5} & 66.0 & 75.3 & 90.1 & 68.4 & 73.9 & 68.9 \\
\midrule
\textsc{Filter} & \textbf{80.1} & \textbf{82.6} & \textbf{81.6} & \textbf{83.5} & \textbf{76.2} & \textbf{83.9} & \textbf{93.8} & \textbf{71.4} & \textbf{74.7} & \textbf{73.4} \\
\bottomrule
\end{tabular}
%\end{adjustbox}
\caption{Results on the test set of XGLUE. \textsc{Filter} achieves new state of the art at the time of submission (Sep. 14, 2020). Note that cross-lingual language generation tasks are not included.
%($\star$) This number is removed as it was obtained by using full training data instead of English training data only, based on communications with the authors.
Leaderboard: \url{https://microsoft.github.io/XGLUE}.}
\label{tbl:xglue_leaderboard}
%\vspace{-1mm}
% We use InterXLM without self-teaching loss for submission whose name is MTDA.
\end{table*}

==> tables/xtreme_leaderboard.tex <==
\begin{table}[!htb]
\centering
%\begin{adjustbox}{scale=0.95,center}
\begin{tabular}{lccccc}
\toprule
Model & Avg & Clf & Str & QA & SR \\
\midrule
XLM             & 55.8 & 75.0 & 65.6  & 43.9 & 44.7 \\
MMTE            & 59.3 & 74.3 & 65.3  & 52.3 & 48.9 \\
mBERT           & 59.6 & 73.7 & 66.3  & 53.8 & 47.7 \\
XLM-R           & 68.2 & 82.8  & 69.0 & 62.3 & 61.6 \\
X-STILTs         & 73.5 & 83.9  & 69.4 & 67.2 & 76.5 \\
VECO$^\dagger$            & 74.8	& 84.7 & 70.4 & 67.2 & 80.5 \\
\midrule
\textsc{Filter}            & \textbf{77.0} & \textbf{87.5} & \textbf{71.9} & \textbf{68.5} & \textbf{84.5} \\
\bottomrule
\end{tabular}
%\end{adjustbox}
\caption{Results on the test set of XTREME. \textsc{Filter} achieves new state of the art at the time of submission (Sep. 8, 2020). For TydiQA-GoldP dataset, we use additional SQuAD v1.1 English training data. The score on question answering is calculated by the average of EM and F1 scores on three datasets. ($\dagger$) indicates unpublished work. Clf: pair sentence classification, Str: structured prediction, SR: sentence retrieval 
%($\star$) This number is removed as it was obtained by using full training data instead of English training data only, based on communications with the authors.
%Leaderboard: \href{https://sites.research.google/xtreme}{https://sites.research.google/xtreme}.
}
\label{tbl:leaderboard}
%\vspace{-3mm}
% We use InterXLM without self-teaching loss for submission whose name is MTDA.
\end{table}
